Xi-Vector Embedding for Speaker Recognition

We present a Bayesian formulation for deep speaker embedding, wherein the xi-vector is the Bayesian counterpart of the x-vector, taking into account the uncertainty estimate. On the technology front, we offer a simple and straightforward extension to the now widely used x-vector. It consists of an auxiliary neural net predicting the frame-wise uncertainty of the input sequence. We show that the proposed extension leads to substantial improvement across all operating points, with a significant reduction in error rates and detection cost. On the theoretical front, our proposal integrates the Bayesian formulation of linear Gaussian model to speaker-embedding neural networks via the pooling layer. In one sense, our proposal integrates the Bayesian formulation of the i-vector to that of the x-vector. Hence, we refer to the embedding as the xi-vector, which is pronounced as /zai/ vector. Experimental results on the SITW evaluation set show a consistent improvement of over 17.5% in equal-error-rate and 10.9% in minimum detection cost.

==> exp_sitw.tex <==
\addtolength{\tabcolsep}{-2pt}  
\begin{table}[t]
%\footnotesize
\caption{Performance comparison of xi-vector embedding with x-vector on the SITW eval set.}
\vspace{-2ex}
\centerline{
\begin{tabular}{l c c c c}
\toprule
& \multicolumn{1}{c}{EER (\%)} & \multicolumn{3}{c}{MinDCF} \\
 %\cmidrule(lr){3-5}
 \midrule
$P_{target}$ & -- & 0.05 & 0.01 & 0.001 \\
\midrule
x-vector ($\mu,\sigma$)     & 2.65   & 0.175    & 0.278   & 0.470\\
xi-vector ($\phi,\sigma$)   & 2.30   & 0.149    & 0.239   & 0.408\\
%\midrule
x-vector ($\mu$)            & 3.23   & 0.227    & 0.362   & 0.555\\
xi-vector ($\phi$)          & 2.18   & 0.152    & 0.248   & 0.431\\ 
\bottomrule
\end{tabular}}
\label{table:sitw} 
\end{table}
\addtolength{\tabcolsep}{2pt}  

\addtolength{\tabcolsep}{-2pt}  
\begin{table}[t]
%\footnotesize
\caption{Ablation analysis of xi-vector.}
\vspace{-2ex}
\centerline{
\begin{tabular}{l c c c c}
\toprule
& \multicolumn{1}{c}{EER (\%)} & \multicolumn{3}{c}{MinDCF} \\
 %\cmidrule(lr){3-5}
 \midrule
$P_{target}$ & -- & 0.05 & 0.01 & 0.001 \\
\midrule
No-Prior ($\phi$)            & 2.43   & 0.164   & 0.268   & 0.444 \\
No-Prior + Isotropic ($\phi$)           & 3.03   & 0.206   & 0.325   & 0.545 \\
No-Prior ($\phi,\sigma$)     & 2.35   & 0.158   & 0.254   & 0.426 \\
No-Prior + Isotropic ($\phi,\sigma$)    & 2.54   & 0.160   & 0.264   & 0.454 \\
\bottomrule
\end{tabular}}
\label{table:ablation} 
\end{table}
\addtolength{\tabcolsep}{2pt}  



==> exp_wideband.tex <==
\addtolength{\tabcolsep}{-2pt}  
\begin{table}[t]
%\footnotesize
\caption{Performance comparison of xi-vector extractor with x-vector.}
\vspace{-2ex}
\centerline{
\begin{tabular}{l c c c c}
\toprule
& \multicolumn{2}{c}{VoxCeleb1-Test} & \multicolumn{2}{c}{SITW-Eval} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& EER (\%) & MinDCF & EER (\%) & MinDCF \\
\midrule
x-vector ($\mu,\sigma$)     & 2.92   & 0.299   & 2.65   & 0.278 \\
xi-vector ($\phi$)          & 2.78   & 0.296   & 2.18   & 0.248 \\ 
\midrule
xi-vector ($\phi,\sigma$)   & 2.71   & 0.312   & 2.30   & 0.239 \\
x-vector ($\mu$)            & 3.44   & 0.305   & 3.23   & 0.362 \\
\bottomrule
\end{tabular}}
\label{table:vox1_sitw} 
\end{table}
\addtolength{\tabcolsep}{2pt}  

\addtolength{\tabcolsep}{-2pt}  
\begin{table}[t]
%\footnotesize
\caption{Ablation analysis of xi-vector.}
\vspace{-2ex}
\centerline{
\begin{tabular}{l c c c c}
\toprule
& \multicolumn{2}{c}{VoxCeleb1-Test} & \multicolumn{2}{c}{SITW-Eval} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& EER (\%) & MinDCF & EER (\%) & MinDCF \\
\midrule
No-Prior ($\phi$)            & 2.88   & 0.277   & 2.43   & 0.268 \\
Isotropic ($\phi$)           & 3.58   & 0.343   & 3.03   & 0.325 \\
No-Prior ($\phi,\sigma$)     & 2.78   & 0.289   & 2.35   & 0.254 \\
Isotropic ($\phi,\sigma$)    & 2.82   & 0.272   & 2.54   & 0.264 \\
\bottomrule
\end{tabular}}
\label{table:ablation} 
\end{table}
\addtolength{\tabcolsep}{2pt}  


